Tensor-Based Reduced-Order Modeling for Optimization-Based Inverse Problems

We develop a tensor reduced-order modeling (TROM) framework for optimization-based inverse problems governed by parameter-dependent dynamical systems. The approach approximates the parameter-to-observation map directly in tensor-train (TT) format using TT-SVD or TT-Cross and integrates it into a regularized nonlinear least-squares formulation. Beyond accelerating forward evaluations, the low-rank tensor structure reformulates the inverse problem in reduced coordinates, assembles Gauss--Newton quantities without forming the full observation-space Jacobian, and minimizes the TROM objective over the discrete parameter grid. This tensor optimization provides either a stand-alone approximate solution or a data-informed initialization for a subsequent Gauss--Newton solve. We study an inverse heat-transfer problem in a heterogeneous medium, where the parameters describe the locations and radii of low-conductivity inclusions, and a FitzHugh--Nagumo parameter-estimation problem with a highly nonconvex landscape. Numerical experiments assess reduced-order model error, measurement noise, regularization, initialization, spatial discretization, and increasing parameter dimension. The results show that TROM reproduces full-order inversion at substantially reduced online cost. They also demonstrate that reduced-coordinate inversion, tensor-based optimization, and appropriate regularization improve robustness in higher-dimensional, noisy, and strongly nonconvex regimes. For the continuous TROM inverse problem, we develop an error-to-inversion analysis. Under local strong convexity of the regularized FOM objective and parametric smoothness of the FOM observation map, the error between the parameters recovered with the full-order model and TROM is bounded by controlled uniform errors in the surrogate map and its Jacobian, together with local FOM and curvature quantities.

==> shared.tex <==
% packages and macros go here
\input{preamble.tex}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{assumption}{Assumption}
\crefname{assumption}{Assumption}{Assumptions}
\newsiamthm{claim}{Claim}
\newsiamremark{fact}{Fact}
\crefname{fact}{Fact}{Facts}

% AM: siamart gives all theorem-like environments a SHARED counter, and cleveref
% keys its reference type off the counter, so \cref/\Cref on a remark or an
% assumption printed "Theorem" (e.g. "covered by Theorem 4.2" for a Remark).
% \crefname/\Crefname alone cannot fix this; each such \label must also carry an
% explicit type, i.e. \label[remark]{rem:...} / \label[assumption]{ass:...}.
\crefname{remark}{Remark}{Remarks}
\Crefname{remark}{Remark}{Remarks}
\Crefname{assumption}{Assumption}{Assumptions}
\Crefname{fact}{Fact}{Facts}
\crefname{claim}{Claim}{Claims}
\Crefname{claim}{Claim}{Claims}


% sets running headers as well as PDF title and authors
\headers{TROM for Inverse Problems}{S.\ Islam, A.\ Mang, and M.\ Olshanskii}

\title{Tensor-Based Reduced-Order Modeling for Optimization-Based Inverse Problems\thanks{Submitted to the editors DATE.
\funding{The work of the authors was partially supported by the National Science Foundation (NSF) under awards DMS-2145845 (AM) and DMS-2309197 (MO and SI). This material is based upon work supported by the NSF under Grant DMS-1929284 while AM was in residence at the Institute for Computational and Experimental Research in Mathematics in Providence, RI, during the ``Stochastic and Randomized Algorithms in Scientific Computing: Foundations and Applications'' semester program. We are grateful for the support of the Research Computing Data Core at the University of Houston.}}}

% authors: full names plus addresses.
\author{Sahidul Islam\thanks{Department of Mathematics, University of Houston, Houston, TX 77204, USA (\email{maolshanskiy@uh.edu}).} \and Andreas Mang\thanks{Department of Mathematics, Tufts University, Medford, MA 02155, USA (\email{andreas.mang@tufts.edu}).} \and Maxim Olshanskii\footnotemark[2]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

%%% Local Variables:
%%% mode:latex
%%% TeX-master: "main"
%%% End:

